Optimal Mixture Weights for Off-Policy Evaluation with Multiple Behavior Policies

Off-policy evaluation is a key component of reinforcement learning which evaluates a target policy with offline data collected from behavior policies. It is a crucial step towards safe reinforcement learning and has been used in advertisement, recommender systems and many other applications. In these applications, sometimes the offline data is collected from multiple behavior policies. Previous works regard data from different behavior policies equally. Nevertheless, some behavior policies are better at producing good estimators while others are not. This paper starts with discussing how to correctly mix estimators produced by different behavior policies. We propose three ways to reduce the variance of the mixture estimator when all sub-estimators are unbiased or asymptotically unbiased. Furthermore, experiments on simulated recommender systems show that our methods are effective in reducing the Mean-Square Error of estimation.

==> alpha_beta.tex <==
\section{$\alpha\beta$ Mixture Estimator for Multiple Behavior Policies}
\subsection{Mixture Estimator with Control Variates}
In MDR, $\forall i,t$, $\mathbb{E}[\bm{\rho}_{i,t-1}V(\bm{s}_{i,t})-\bm{\rho}_{i,t}Q(\bm{s}_{i,t},\bm{a}_{i,t})]=0$. These parts work as control variates in the estimation. If we split them from $\bm{V}_{i,t}$ and optimize mixture weights of them, we may get better results. Like in section \ref{sec:nm}, we first define mixture estimator with control variates for the estimators.
\begin{definition}
	Given $M*T$ estimators $\hat{V}_{i,t}$, $M*T$ estimators $\hat{W}_{i,t}$, $M*T$ variables $\alpha_{i,t}$ and $M*T$ variables $\beta_{i,t}$, if 
	\begin{itemize}
		\item $\forall i,t$, $\mathbb{E}[\hat{V}_{i,t}]=V_t$ and $\mathbb{E}[\hat{W}_{i,t}]=0$;
		\item $\forall t$, $\sum_{i=1}^M\alpha_{i,t}=1$
	\end{itemize}
then $\hat{V}_{\alpha,\beta}=\sum_{i=1}^M\sum_{t=0}^T(\alpha_{i,t}\hat{V}_{i,t}+\beta_{i,t}\hat{W}_{i,t})$ is called mixture estimator with control variates for the estimators.
\end{definition}
We can easily verify that $\hat{V}_{\alpha,\beta}$ is unbiased for $V=\sum_{t=0}^TV_t$. Now we would like to minimize the variance of such estimator by optimizing the mixture weights.
\subsection{Optimal Mixture Weights for Mixture Estimator with Control Variate}
The following proposition derives optimal mixture weights for mixture estimator with control variates.
\begin{proposition}
\label{prop:5}
	Given $M*T$ estimators $\hat{V}_{i,t}$ and $M*T$ estimators $\hat{W}_{i,t}$, if
	\begin{itemize}
		\item  $\forall i_1,i_2,t_1,t_2$, if $i_1\neq i_2$, then $\hat{V}_{i_1,t_1}$ and $\hat{V}_{i_2,t_2}$ are independent, $\hat{W}_{i_1,t_1}$ and $\hat{W}_{i_2,t_2}$ are independent, $\hat{V}_{i_1,t_1}$ and $\hat{W}_{i_2,t_2}$ are independent;
		\item $\forall i,t$, $\mathbb{E}[\hat{V}_{i,t}]=V_t$ and $\mathbb{E}[\hat{W}_{i,t}]=0$;
	\end{itemize}
	then the mixture weights that minimize the variance of mixture estimator with control variates for the estimators are $\overrightarrow{\alpha}_i^*=H_{i,11}(\sum_{i'=1}^MH_{i',11})^{-1}\overrightarrow{e}$, $\overrightarrow{\beta}_i^*=H_{i,21}(\sum_{i'=1}^MH_{i',11})^{-1}\overrightarrow{e}$, where $\left(\begin{matrix}H_{i,11}&H_{i,12}\\H_{i,21}&H_{i,22}\end{matrix}\right)$ is the precision matrix of $[\hat{V}_{i,0}, \hat{V}_{i,1}, ..., \hat{V}_{i,t}, \hat{W}_{i,0}, \hat{W}_{i,1}, ..., \hat{W}_{i,t}]^T$.
\end{proposition}
See Appendix \ref{ap:pr5} for proof. We call this estimator $\alpha\beta$ mixture estimator. In OPE, it can be applied to reduce the variance of DR and WDR. 
 
\subsection{$\alpha\beta$ Mixture Doubly Robust Estimation and $\alpha\beta$ Mixture Weighted Doubly Robust Estimation}
To construct $\alpha\beta$ mixture estimator for DR, we formulate the estimators as $\hat{V}_{i,t}=\frac{1}{n_i}\sum_{j=1}^{n_i}\hat{V}_{i,j,t}$ and $\hat{W}_{i,t}=\frac{1}{n_i}\sum_{j=1}^{n_i}\hat{W}_{i,j,t}$. Then the estimated mixture weights are $\overrightarrow{\alpha}_i=k_i\hat{H}_{i,11}(\sum_{i'=1}^Mk_{i'}\hat{H}_{i',11})^{-1}\overrightarrow{e}$, $\overrightarrow{\beta}_i=k_i\hat{H}_{i,21}(\sum_{i'=1}^Mk_{i'}\hat{H}_{i',11})^{-1}\overrightarrow{e}$, where $\hat{H}$ are components of empirical precision matrix of $[\bm{V}_{i,0},\bm{V}_{i,1},...,\bm{V}_{i,T},\bm{W}_{i,0},\bm{W}_{i,1},...,\bm{W}_{i,T}]^T$ estimated by samples. We can prove that with these weights, the mixture estimator with control variates is strongly consistent for V. We call this estimator $\alpha\beta$ Mixture Doubly Robust estimator($\alpha\beta$MDR).

To construct $\alpha\beta$ mixture estimator for WDR, we need to estimate the covariance between $\hat{W}_{i,t_1}$ and $\hat{W}_{i,t_2}$, and the covariance between $\hat{V}_{i,t_1}$ and $\hat{W}_{i,t_2}$. These can be done by setting proper variables like in section \ref{sub:43}. We call this estimator $\alpha\beta$ Mixture Weighted Doubly Robust estimator($\alpha\beta$MWDR).


==> mixture.tex <==
\section{Mixture Estimator for Multiple Behavior Policies}
\subsection{Mixture Estimators for Reinforcement Learning}
By the split view of estimation, we can build another mixture estimator for the MDP $\hat{V}_{MIXT} = \sum_{i=1}^M\sum_{t=0}^{T}\alpha_{i,t}\hat{V}_{i,t}$, where $\forall t\in[0,T]$, $\sum_{i=1}^M\alpha_{i,t}=1$ and $\hat{V}_{i,t}$ is the value estimator at horizon $t$ by the $i$-th estimator. Denote the mean reward of the MDP at horizon $t$ by $V_t$, we give the following proposition to optimize such mixture weights.
\begin{proposition}
\label{prop:3}
	Denote the covariance matrix of $[\hat{V}_{i,0},\hat{V}_{i,1},...,\hat{V}_{i,T}]$ by $\Sigma_i$. If 
	\begin{itemize}
		\item $\forall i_1,i_2,t_1,t_2$, if $i_1\neq i_2$, then $\hat{V}_{i_1,t_1}$ and $\hat{V}_{i_2,t_2}$ are independent;
		\item $\forall i\forall t$, $\hat{V}_{i,t}$ is unbiased for $V_t$;
		\item $\forall i\ \Sigma_i$ is positive definite;
	\end{itemize}
	then $V_{MIXT}$ is unbiased and the mixture weights that minimize variance of $\hat{V}_{MIXT}$ are $\overrightarrow{\alpha}_i^*=\Sigma_i^{-1}(\sum_{i'=1}^M\Sigma_{i'}^{-1})^{-1}\overrightarrow{e}$, where $\overrightarrow{\alpha}_i^*=[\alpha_{i,0},\alpha_{i,1},...,\alpha_{i,T}]^{T}$ and $\overrightarrow{e}$ is $[1,1,...,1]^T$. Moreover, $\mathbb{V}[\hat{V}_{MIXT}]\le\mathbb{V}[\hat{V}_{MIX}]$.
\end{proposition}
See appendix \ref{ap:pr3} for proof. The assumption of positive definite is not hard to reach in real world problems. If the reward is constant at some horizon, we can simply remove it from our formula and still get a positive definite covariance matrix. To understand $\hat{V}_{MIXT}$, we consider one sample of data. In $\hat{V}_{MIX}$, different parts of the data are combined. But in $\hat{V}_{MIXT}$, different parts of the data are split and may be assigned different weights. 
\subsection{Mixture Importance Sampling and Mixture Doubly Robust Estimation}
For IS and DR, it is direct to split the estimation by $t$. Taking DR for example, we can make $\hat{V}_{i,t}=\frac{1}{n_i}\sum_{j=1}^{n_i}\hat{V}_{i,j,t}=\frac{1}{n_i}\sum_{j=1}^{n_i}\gamma^t\left(\rho_{i,j,t-1}\hat{V}(s_{i,j,t})+\rho_{i,j,t}(r_{i,j,t}-\hat{Q}(s_{i,j,t},a_{i,j,t}))\right)$. The optimal mixture weights can be written as $\overrightarrow{\alpha}_i^*=(\frac{\tilde{\Sigma}_{i}}{k_i})^{-1}(\sum_{i'=1}^M(\frac{\tilde{\Sigma}_{i'}}{k_{i'}})^{-1})^{-1}\overrightarrow{e}$, where $\tilde{\Sigma}_{i}$ is the covariance matrix of $[\bm{V}_{i,0},\bm{V}_{i,1},...,\bm{V}_{i,T}]$. We can directly estimate $\tilde{\Sigma}_{i}$ by samples and construct Mixture Importance Sampling(MIS) and Mixture Doubly Robust estimation(MDR). We give the following proposition to guarantee the convergence of MIS and MDR.
\begin{proposition}
	Denote the estimation of $\tilde{\Sigma}_{i}$ by $\hat{\Sigma}_{i}$. If
	\begin{itemize}
		\item $\forall i_1,i_2,t_1,t_2$, if $i_1\neq i_2$, then $\hat{V}_{i_1,t_1}$ and $\hat{V}_{i_2,t_2}$ are independent;
		\item $\forall i$, $\hat{\Sigma}_{i}$ is strongly consistent for $\tilde{\Sigma}_{i}$;
		\item $\forall i,t$, $\hat{V}_{i,t}$ is strongly consistent for $V_t$;
	\end{itemize}

	then the empirical estimation $\hat{V}_{MIXT}=\sum_{i=1}^M{\hat{\alpha}}_{i}^T\overrightarrow{V}_i$, where ${\hat{\alpha}}_i=(\frac{\hat{\Sigma}_{i}}{k_i})^{-1}(\sum_{i'=1}^M(\frac{\hat{\Sigma}_{i'}}{k_{i'}})^{-1})^{-1}\overrightarrow{e}$ and $\overrightarrow{V}_i=[\hat{V}_{i,0},\hat{V}_{i,1},...,\hat{V}_{i,T}]^T$, is strongly consistent for $V$.

\end{proposition}
See Appendix \ref{ap:pr4} for proof. The estimators for covariance matrixes as well as values are all strongly consistent. So MIS and MDR are strongly consistent estimators. 
\subsection{Mixture Weighted Importance Sampling and Mixture Weighted Doubly Robust Estimation}
\label{sub:43}
For WIS and WDR, we can also split values by t like IS and DR. To estimate the covariance matrix, we need to estimate the covariance between $\hat{V}_{i,t_1}$ and $\hat{V}_{i,t_2}$. Define $\hat{V}_{i,t}=\nu_{i,t}+\omega_{i,t}=\frac{\sum_{j=1}^{n_i}\hat{X}_{i,j,t}}{\sum_{j=1}^{n_i}\hat{W}_{i,j,t}}+\frac{\sum_{j=1}^{n_i}\hat{Z}_{i,j,t}}{\sum_{j=1}^{n_i}\hat{Y}_{i,j,t}}$. The formulation of covariance would be $Cov_{i,t_1,t_2}=\sum_{j=1}^{n_i}\left(\frac{\hat{X}_{i,j,t_1}-\nu_{i,t_1}\hat{W}_{i,j,t_1}}{\sum_{k=1}^{n_i}\hat{W}_{i,k,t_1}}+\frac{\hat{Z}_{i,j,t_1}-\omega_{i,t_1}\hat{Y}_{i,j,t_1}}{\sum_{k=1}^{n_i}\hat{Y}_{i,k,t_1}}\right)\left(\frac{\hat{X}_{i,j,t_2}-\nu_{i,t_2}\hat{W}_{i,j,t_2}}{\sum_{k=1}^{n_i}\hat{W}_{i,k,t_2}}+\frac{\hat{Z}_{i,j,t_2}-\omega_{i,t_2}\hat{Y}_{i,j,t_2}}{\sum_{k=1}^{n_i}\hat{Y}_{i,k,t_2}}\right)$. Note that $n_i Cov_{i,t_1,t_2}$ is also strongly consistent for a constant. See Appendix \ref{ap:csw}. So similar to Section \ref{sec:33}, we can build a strongly consistent estimator for V. For WIS, we let $\hat{X}_{i,j,t}=\gamma^t\rho_{i,j,t}r_{i,j,t}$, $\hat{W}_{i,j,t}=\rho_{i,j,t}$ and $\hat{Z}_{i,j,t}=0$. For WDR, we set $\hat{X}_{i,j,t}=\gamma^t\rho_{i,j,t}(r_{i,j,t}-\hat{Q}(s_{i,j,t},a_{i,j,t}))$, $\hat{W}_{i,j,t}=\rho_{i,j,t}$, $\hat{Z}_{i,j,t}=\gamma^t\rho_{i,j,t-1}\hat{V}(s_{i,j,t})$ and $\hat{Y}_{i,j,t}=\rho_{i,j,t-1}$. We call the estimators Mixture Weighed Importance Sampling(MWIS) and Mixture Weighted Doubly Robust estimation(MWDR).

\subsection{Problems of Mixture Doubly Robust Estimation}
Regardless of the variance reduction compared with NMDR, there are problems in MDR. Adding up the MDR estimators for the $i$-th policy, we will get $\hat{V}_{i,MDR}=\sum_{j=1}^{n_i}\sum_{t=0}^T\alpha_{i,t}\gamma^t(\rho_{i,j,t-1}\hat{V}(s_{i,j,t})+\rho_{i,j,t}(r_{i,j,t}-\hat{Q}(s_{i,j,t},a_{i,j,t})))]$. In the original Doubly Robust estimators, $Q$ is the control variate for all the rewards following the current state and action, which means $\mathbb{E}[\bm{\rho}_{i,t}Q(\bm{s}_{i,t},\bm{a}_{i,t})]\approx\mathbb{E}[\sum_{\tau=t}^T\gamma^{\tau-t}\bm{\rho}_{i,\tau}\bm{r}_{i,\tau}]$. However, in MDR, rewards at different time may be assigned different weights and $\mathbb{E}[\alpha_{i,t}\bm{\rho}_{i,t}Q(\bm{s}_{i,t},\bm{a}_{i,t})]$ can be far from $\mathbb{E}[\sum_{\tau=t}^T\alpha_{i,\tau}\gamma^{\tau-t}\bm{\rho}_{i,\tau}\bm{r}_{i,\tau}]$. This means that $Q$ may not be the best control variate for mixing DR estimators. To optimize MDR, we then propose to further split Doubly Robust estimators.


==> naive_mixture.tex <==
\section{Naive Mixture Estimators for Multiple Behavior Policies}
\label{sec:nm}
\subsection{Naive Mixture Estimator}
We first define the mixture estimator of multiple estimators.
\begin{definition}
	Given $M$ unbiased estimators $\hat{V}_1,\hat{V}_2,...,\hat{V}_M$ of a value $V$ and M variables $\alpha_1,...,\alpha_M$, if $\sum_{i=1}^M\alpha_i=1$, then $\hat{V}_{\alpha}=\sum_{i=1}^M\alpha_i\hat{V}_i$ is called a mixture estimator of the M estimators.
\end{definition}
It is not hard to prove that mixture estimators are unbiased for $V$. We further show the optimal mixture weights of multiple estimators by giving the following theorem.
\begin{theorem}
\label{theo:t1}
	Given $M$ unbiased and independent estimators $\hat{V}_1,\hat{V}_2,...,\hat{V}_M$ of a value $V$, the mixture estimator of them with the minimal variance is $\hat{V}_{MIX}=\sum_{i=1}^M\alpha_i^*\hat{V}_i$, where $ \alpha_i^*=\frac{1}{\mathbb{V}[\hat{V}_i]\sum_{i'=1}^M\frac{1}{\mathbb{V}[\hat{V}_{i'}]}}$. The minimal variance is $\frac{1}{\sum_{i=1}^M\frac{1}{\mathbb{V}[\hat{V}_i]}}$.
\end{theorem}

See Appendix \ref{ap:th1} for proof. Theorem \ref{theo:t1} is the general case for Section 6 of \citeinline{Aman2017EffectiveEva} as well as the basis of Fixed Effect Model in Meta Analysis\cite{MetaAnalysis}. We call this estimator naive mixture estimator because it does not consider the properties of reinforcement learning.

\subsection{Naive Mixture Importance Sampling and Naive Mixture Doubly Robust Estimation}
Naive mixture estimators can be directly applied to mix IS and DR estimators. If we compute the $i$-th estimator as $\hat{V}_i=\frac{1}{n_i}\sum_{j=1}^{n_i}\hat{V}_{i,j}$ where $\hat{V}_{i,j}$ denotes the estimation for the $j$-th data of the $i$-th estimator, then the optimal mixture weights for Naive Mixture Importance Sampling(NMIS) or Naive Mixture Doubly Robust estimation(NMDR) are $\alpha_i^*=\frac{k_i}{\mathbb{V}[\bm{V}_{i}]\sum_{i'=1}^M\frac{k_{i'}}{\mathbb{V}[\bm{V}_{i'}]}}$, where $\bm{V}_i$ is the random variable of $\hat{V}_{i,j}$. Note we can also estimate $\mathbb{V}[\bm{V}_{i}]$ by samples. To guarantee the strong consistency for NMIS and NMDR, we give the following proposition:
\begin{proposition}
	If $\forall i$, $Var_i$ and $\hat{V}_i$ are strongly consistent estimators for $\mathbb{V}[\bm{V}_{i}]$ and $V$, then $\hat{V}_{MIX}=\frac{1}{\sum_{i=1}^M \frac{k_i}{Var_i}}\sum_{i=1}^M\frac{k_i\hat{V}_i}{Var_i}$ is strongly consistent for $V$.
\end{proposition}
See Appendix \ref{ap:pr1} for proof. Because Assumption \ref{ass:1} and Assumption \ref{ass:2} hold, $Var_i$ and $\hat{V}_i$ are both strongly consistent. Therefore, NMIS and NMDR are strongly consistent for $V$.
\subsection{Naive Mixture Weighted Importance Sampling and Naive Mixture Weighted Doubly Robust Estimation}
\label{sec:33}
Previous works of WIS and WDR combines data from different behavior policies together. We can formulate such weighted estimators as $\hat{V}_{W}=\sum_{t=0}^T\frac{\sum_{i=1}^M\sum_{j=1}^{n_i}\hat{Y}_{i,j,t}}{\sum_{i=1}^M\sum_{j=1}^{n_i}\hat{X}_{i,j,t}}$, where $\hat{X}_{i,j,t}$ are samples of $\bm{X}_{i,t}$ and $\hat{Y}_{i,j,t}$ are samples of $\bm{Y}_{i,t}$. But in this paper, we split data by behavior policy. The $i$-th split weighted estimator is $\hat{V}_i=\sum_{t=0}^T\hat{\theta}_{i,t}=\sum_{t=0}^T\frac{\sum_{j=1}^{n_i}\hat{Y}_{i,j,t}}{\sum_{j=1}^{n_i}\hat{X}_{i,j,t}}$. To apply naive mixture estimators, we need to estimate the variance of each $\hat{V}_i$. 

By Delta Method\cite{Owen2013MonteCarlo}, we approximate $\mathbb{V}[\hat{V}_i]$ by $Var_i=\sum_{j=1}^{n_i}\left(\sum_{t=0}^T\frac{\hat{Y}_{i,j,t}-\hat{\theta}_{i,t}\hat{X}_{i,j,t}}{\sum_{k=1}^{n_i}\hat{X}_{i,k,t}}\right)^2$. We can also prove that $n_i*Var_i$ is strongly consistent for a constant $E_i=\mathbb{E}[\left(\sum_{t=0}^T\frac{\bm{Y}_{i,t}-\theta_{i,t}\bm{X}_{i,t}}{\mathbb{E}[\bm{X}_{i,t}]}\right)^2]$. See Appendix \ref{ap:vsw}. If we define the mixture weights for naive mixture weighted estimators as $\hat{\alpha}_i=\frac{1}{Var_i\sum_{i=1}^M\frac{1}{Var_i}}$, then the naive mixture estimators $\hat{V}_{NMW}=\frac{1}{\sum_{i=1}^M\frac{1}{Var_i}}\sum_{i=1}^M\frac{\hat{V}_i}{Var_i}$ for split WIS and split WDR are strongly consistent for V. To show the effectiveness of such mixture estimators, we give the following proposition:
\begin{proposition}
	If the error of Delta Method is neglected, $\mathbb{E}[\bm{X}_{i,t}]$ does not depend on i and t, and $\mathbb{E}[\bm{Y}_{i,t}]$ does not depend on i, then $\mathbb{V}[\hat{V}_{NMW}]\le\mathbb{V}[\hat{V}_W]$.
\end{proposition}

See Appendix \ref{ap:pr2} for proof. In WIS and WDR, $\bm{X}_{i,t}$ are importance ratios so $\mathbb{E}[\bm{X}_{i,t}]$ do not depend on $i$ and $t$. In addition, $\bm{Y}_{i,t}$ are unbiased for the mean reward at $t$ so $\mathbb{E}[\bm{Y}_{i,t}]$ do not depend on $i$. Thus naive mixture weighted estimators will not have larger variance than the vanilla weighted estimators. 

We now construct Naive Mixture Weighted Importance Sampling(NMWIS). If we let $\hat{X}_{i,j,t}=\rho_{i,j,t}$ and $\hat{Y}_{i,j,t}=\gamma^t\rho_{i,j,t}r_{i,j,t}$, then the $i$-th split weighted estimator is $\hat{V}_i=\sum_{t=0}^T\hat{\theta}_{i,t}=\sum_{t=0}^T\sum_{j=1}^{n_i}\gamma^tw_{i,j,t}r_{i,j,t}$, where $w_{i,j,t}=\frac{\rho_{i,j,t}}{\sum_{k=1}^{n_i}\rho_{i,k,t}}$. And the $i$-th variance estimator is $Var_i=\sum_{j=1}^{n_i}(\sum_{t=0}^Tw_{i,j,t}(\gamma^tr_{i,j,t}-\hat{\theta}_{i,t}))^2$. Similarly, we can also construct Naive Mixture Weighted Doubly Robust estimation(NMWDR).

A key observation which motivates the following parts is that each original estimator consists of a summation over time $t$. If we further split each original estimator to $(T+1)$ estimators, can we optimize the mixture weights to the $(T+1)M$ split estimators? 
